SparseDM: Toward Sparse Efficient Diffusion Models

Diffusion models represent a powerful family of generative models widely used for image and video generation. However, the time-consuming deployment, long inference time, and requirements on large memory hinder their applications on resource constrained devices. In this paper, we propose a method based on the improved Straight-Through Estimator to improve the deployment efficiency of diffusion models. Specifically, we add sparse masks to the Convolution and Linear layers in a pre-trained diffusion model, then transfer learn the sparse model during the fine-tuning stage and turn on the sparse masks during inference. Experimental results on a Transformer and UNet-based diffusion models demonstrate that our method reduces MACs by 50% while maintaining FID. Sparse models are accelerated by approximately 1.2x on the GPU. Under other MACs conditions, the FID is also lower than 1 compared to other methods.

==> ethics_statement.tex <==
\section{Ethics Statement}

While our motivation is to make diffusion models generate images faster, we also recognize the ethical implications inherent in model pruning, as sparse optimization may introduce unintended biases. There are differences between traditional evaluation metrics (such as FID scores) and human eye evaluation, and optimization for FID may not capture subtle deviations in human vision. In addition to performance improvements to diffusion models, we are also actively focusing on the ethical aspects of AI deployment. We are committed to preventing the spread of content that may have a negative social impact. Prevent unintended consequences by acknowledging the limitations of FID indicators.
